Election Manipulation on Social Networks: Seeding, Edge Removal, Edge Addition

We focus on the election manipulation problem through social influence, where a manipulator exploits a social network to make her most preferred candidate win an election. Influence is due to information in favor of and/or against one or multiple candidates, sent by seeds and spreading through the network according to the independent cascade model. We provide a comprehensive study of the election control problem, investigating two forms of manipulations: seeding to buy influencers given a social network, and removing or adding edges in the social network given the seeds and the information sent. In particular, we study a wide range of cases distinguishing for the number of candidates or the kind of information spread over the network. Our main result is positive for democracy, and it shows that the election manipulation problem is not affordable in the worst-case except for trivial classes of instances, even when one accepts to approximate the margin of victory. In the case of seeding, we also show that the manipulation is hard even if the graph is a line and that a large class of algorithms, including most of the approaches recently adopted for social-influence problems, fail to compute a bounded approximation even on elementary networks, as undirected graphs with every node having a degree at most two or directed trees. In the case of edge removal or addition, our hardness results also apply to the basic case of social influence maximization/minimization. In contrast, the hardness of election manipulation holds even when the manipulator has an unlimited budget, being allowed to remove or add an arbitrary number of edges.

==> costantBound.tex <==
Since pessimistic ranking revision function is not least-candidate manipulable for three candidates, then Theorem~\ref{thm:inapprox} applies, and thus we have the following.
\begin{proposition}
\label{prop:pessimistic3}
 For every $\rho >0$ even depending on the size of the problem, unless $\mathsf{P} = \mathsf{NP}$ there is no poly-time algorithm returning a $\rho$-approximation to the election problem with pessimistic ranking revision function, even for only three candidates.
\end{proposition}

By focusing on optimistic ranking revision function, we have that $\ell$ negative messages about $c_1, \ldots, c_\ell$ are sufficient to make $c_0$ first, regardless of the initial ranking.
Hence, we can apply Theorem~\ref{thm:approx} with $\tau = \ell$, and we have the following.
\begin{proposition}
 \label{prop:optimistic3}
 There is a greedy poly-time algorithm that returns a $\rho$-approximation to the election control problem with optimistic ranking revision function for three candidates, with
 $$
  \rho = \frac{B - \ell + 1}{2\ell B}\left(1-\frac{1}{e}\right).
%   \approx \frac{1}{4} \left(1-\frac{1}{e}\right).
 $$
 The result holds even if only negative influences are allowed.
\end{proposition}

Differently from the optimistic ranking revision function, for the score-based one, negative message only are not sufficient for make $c_0$ first when she is last in the initial ranking. However, when there are only three available candidates, it is possible to ensure that $c_0$ reaches the first position with only three messages, namely $(+,-,-)$. Hence, from Theorem~\ref{thm:approx} we achieve the following.
\begin{proposition}
	\label{prop:score3}
	There is a greedy poly-time algorithm that returns a $\rho$-approximation to the election control problem with score-based ranking revision function for three candidates, with
	$$
	\rho = \frac{B - 2}{6B}\left(1-\frac{1}{e}\right) \approx \frac{1}{6} \left(1-\frac{1}{e}\right).
	$$
\end{proposition}

 Moreover, differently from the optimistic ranking revision function, for the score-based one the approximation guarantee ceases to hold if only negative influences are allowed. Indeed, in this case there is no way for the last ranked candidate to become the first one, and thus Theorem~\ref{thm:inapprox} holds.
\begin{proposition}
	\label{prop:score3neg}
	For every $\rho >0$ even depending on the size of the problem, unless $\mathsf{P} = \mathsf{NP}$, there is no poly-time algorithm returning a $\rho$-approximation to the election problem with score-based ranking revision function if only negative influences are allowed, even for only three candidates.
\end{proposition}

We show that, whereas an approximation algorithm exists for the optimistic ranking revision function with only negative influence, this result does not carry on to the case that only positive influence is allowed. Indeed, in this case, there is no way to raise the rank of the last candidate up to the first position, and thus Theorem~\ref{thm:inapprox} applies.

\begin{proposition}
\label{prop:opt3pos}
 For every $\rho >0$ even depending on the size of the problem, unless $\mathsf{P} = \mathsf{NP}$, there is no polynomial time algorithm returning a $\rho$-approximation to the election problem if only positive influences are allowed, even for only three candidates and optimistic ranking revision function.
\end{proposition}

% \paragraph{Different tie-breaking rule}
% 
%  However, while for the pessimistic TBR also considering only negative influences does not generate ties and then the formerly obtained results still hold, things change for the optimistic TBR. Indeed, with this tie-breaking rule, it is possible to obtain a constant bound even with only negative influences.
%  
% \begin{theorem}
% 	If the optimistic TBR holds, greedily optimizing f(S) with $\frac{k}{2}$ seeds with $I(s_i)=(\cdot,-,-) , \forall s_i \in S$, provides
% 	$$\mathcal M(S) \ge \frac{1-\frac{1}{k}}{4}\left( 1-\frac{1}{e}\right) \mathcal M(S^*)$$
% \end{theorem}
% 
% It can be noted that, if the optimistic TBR holds, it is enough to place two seeds per node. Therefore the bound is tighter than the one obtained for the standard TBR with positive and negative influences. Then it can be stated that, if only negative influences spread and the optimistic TBR holds, the problem is APX-complete.
% 
% We consider now the case in which both positive and negative influence spreads for the three-candidates case. It is clear that, if the optimistic TBR holds, the problem is still APX-complete. Otherwise, if the pessimistic TBR holds, no constant bound can be defined, in particular the one obtained for the standard TBR is no more valid since $I(v)=(+,-,-)$ is not enough to make $v$ vote for $c_*$. Thus, supposing to be in a situation in which $c_*$ is always ranked as first or as third, the only way of dealing with the problem is focusing on the first two preferences of each node. In the proof of the inapproximability for the four candidates case, we actually faced the same scenario after having proved that $c_3$ and $c_*$ should neither gain or loose votes. Here we suppose to remove $v_A$ and $v_B$ and that the cardinality of $G_2^1$ is $|G_2^1|= 2(m+n) + m - h + 1$. Nevertheless, the proof still partially holds and it can be stated that also in the three candidates scenario with positive and negative influences, according to the pessimistic tie-breaking rule, computing $\max_{|S| \le k} M(S)$ in election is not in APX. 
% 
% Moreover, also in this setting, we can employ an "enlarging" technique. In fact suppose that every node of the three-candidates mapping (without $v_A$ and $v_B$) becomes a completely connected subgraph of size $h m n$ and, instead of having $|G_2^1|=h m n \: (2(m+n) + m - h + 1)$, the cardinality of $G_2^1$ is $|G_2^1|=h m n \: (2(m+n) + m - h + 1) - h$ and there exist $h$ disconnected nodes with preferences ranked as $c_1 > c_2 > c_*$. Then, if SET COVER is satisfiable, $\mathcal M(S^*) = h m n$, while if it is not satisfiable, $\mathcal M(S^*) = h$. Since the instance dimension is $O(hmn(m+n))$, we can state that in the three-candidate case, when the pessimistic TBR holds, the problem is not in \LogAPX.
% 
% An equivalent reasoning may be adapted to the four-candidates scenario, which is a generalization of the previous case. Therefore, also with four candidates, the problem is not in \LogAPX. It can be proved that this is actually valid for both the optimistic and the pessimistic TBR.

